Deep Proximal Learning for High-Resolution Plane Wave Compounding

Plane Wave imaging enables many applications that require high frame rates, including localisation microscopy, shear wave elastography, and ultra-sensitive Doppler. To alleviate the degradation of image quality with respect to conventional focused acquisition, typically, multiple acquisitions from distinctly steered plane waves are coherently (i.e. after time-of-flight correction) compounded into a single image. This poses a trade-off between image quality and achievable frame-rate. To that end, we propose a new deep learning approach, derived by formulating plane wave compounding as a linear inverse problem, that attains high resolution, high-contrast images from just 3 plane wave transmissions. Our solution unfolds the iterations of a proximal gradient descent algorithm as a deep network, thereby directly exploiting the physics-based generative acquisition model into the neural network design. We train our network in a greedy manner, i.e. layer-by-layer, using a combination of pixel, temporal, and distribution (adversarial) losses to achieve both perceptual fidelity and data consistency. Through the strong model-based inductive bias, the proposed architecture outperforms several standard benchmark architectures in terms of image quality, with a low computational and memory footprint.

==> Deep Proximal Learning for High-Resolution Plane Wave Compounding/chapters/acknowledgement.tex <==
\section*{Acknowledgment}

The authors would like to thank Dr. Elik Aharoni, Ronnie Rosen, and Oded Drori for their guidance and help in collecting the \textit{in-vivo} data. We would also like to thank the Weizmann Institute of Science for accommodating a visit in the spirit of international collaboration.  

==> Deep Proximal Learning for High-Resolution Plane Wave Compounding/chapters/conclusions.tex <==
\section{Conclusions}\label{chapter:conclusion}


We proposed a model-based deep neural architecture for high-resolution plane wave compounding, incorporating strong physics-based inductive biases. Following the unfolding approach, we observe that the proposed network out-performs several benchmarks by approximately 5\%, using the MAE metric.  

Perceptually, the proximal network produces images with enhanced fidelity, containing high structural resolution and contrast, as shown in Figs. \ref{fig:compare_all_res} and \ref{fig:compare_all_mods}. We also derive a high quality prediction on the point scatterers as seen in the second row of Fig. \ref{fig:compare_all_res}, with a high degree of side-lobe suppression, resolution, and contrast. The same is confirmed using a 1D lateral profile of the point scatterers. We also further demonstrate that it is beneficial to include a significant number of \textit{in-silico} samples in the training of the network, and that increasing the number of folds beyond 5 does not necessarily lead to better performance, which is in line with other works that have trained unfolded networks \cite{solomon2019deep}. Replacing the proximal operator with other potential candidates is a great avenue for further research, along with enhanced data augmentation.  

While it is typically infeasible to make use of MV beamforming in real-time applications, we have presented a neural architecture that can greatly enhance the resolution and contrast of ultrasound images, over DAS beamformed images, with great potential for real-time applications. We achieve the above results with a relatively low parameter count when compared to other architectures. We conclude that the model-based approach proposed here can produce better results under a comparatively small computational foot-print. 

% From Table \ref{table:results}, we can also show that the unfolded proximal gradient scheme  
% As a result, the presented network also manages to perform very well when the beam profiles are compared between the ground truth and the regularly compounded point scatterer image.

% We achieve the above results without a loss in temporal resolution, and a reduction in the volume of data (number of PW transmits) required by a factor of 25, down from 75 PW transmits to 3 PW transmits. We can also conclude that the model based approach proposed here can produce better results under a comparatively small computational foot-print. 

% As a result, we also obtain a network that has excellent performance on synthetic point scatterer data. When such techniques are implemented within a greedy framework, we can achieve results that can obtain high resolution and better contrast. 

% While the network presented in this paper is quite sensitive to the features in the input images, augmenting the training data could allay this problem. 

% This is achieved in addition to promoting the physical validity of the predictions made by the network, due to the embedded physical measurement model.


% We expect the inference times to be perfectly sufficient for real-time applications, when optimised for deployment. 

%Using the validation set, the Unfolded Proximal Gradient Scheme achieves a PSNR of 18.01 $\pm$ 1.43 dB, compared to 15.49 $\pm$ 4.42 dB from a UNet with a similar number of parameters. 

==> Deep Proximal Learning for High-Resolution Plane Wave Compounding/chapters/data_acquisition.tex <==
\section{Data Acquisition}\label{chapter:data_acquisition}

%\begin{figure*}[t!]
% trim={<left> <lower> <right> <upper>}
%    \centering
%    \includegraphics[trim={4cm 7.9cm 18cm 0},clip,width=\textwidth]{images/train.pdf}
%    \caption{The graphic displays the flow of data and loss in the training loop. Pink indicates the flow of loss values, and black indicates the flow of data, from input to output. The green blocks indicate the unfoldings of the prox network, upto $K$ unfoldings. The block to the right hand side of the image with a neuron indicates the discriminator. And as we need frame \textit{t-1} and \textit{t} for the calculation of all loss terms, the graphic also displays the training loop across frames in an acquisition.}
%    \label{fig:train}
%\end{figure*}


% \begin{figure*}[t!]
%     \centering
%     \includegraphics[trim={6cm 4cm 10cm 8cm},clip,width=\textwidth]{images/greedy.pdf}
%     \caption{The figure above describes the process of implementing greedy training in the training of the unfolded proximal network. In the first iteration, we only consider and train the first and the last folds. After which, we add an intermediary fold and freeze the first layer during training. The process is continued until the full network has been trained.}
%     \label{fig:greedy}
% \end{figure*}

For this study we acquired both \textit{in-vivo} and \textit{in-silico} data. The \textit{in-vivo} data from 2 healthy volunteers was acquired using a Vantage system (Verasonics Inc., WA, USA), with the L11-4v and the L11-5v transducers. It was collected across 3 separate scan sessions, containing scans of the carotid artery in various alignments, muscle tissue, and the Achilles tendon. The \textit{in-silico} data consists of 20 randomly spaced point scatterers, at random distances from each other, created using the Verasonics simulation mode. Thirty of the \textit{in-silico} images also contained simulated speckle, made using 10,000 point scatterers of low reflectivity. 

An overview of the driving schemes and imaging parameters for both the LR input data and HR target data is given in Table~\ref{table:parameters}. The LR inputs (using 3 plane waves with a center frequency of 4 MHz) and HR targets (using 75 plane waves with a center frequency of 12 MHz) were acquired in successive frames. All 75 transmissions are equally spaced between the steering angles of $-18^{o}$ and $18^{o}$. All channel data was converted to beamformed RF using pixel-based beamforming. To further improve image quality in the HR acquisitions, we performed minimum variance (MV) beamforming, as opposed to regular delay-and-sum (DAS) for the LR acquisitions. To reduce motion between our input-target pairs, we gather the data using an acquisition sequence that gathers the low frequency image in the first frame, and the high frequency image in the subsequent frame.

\begin{table*}[t!]
\caption{Parameters of the US probes, driving schemes, and beamforming methods for the high-resolution (HR) targets and low-resolution (LR) inputs.}
\centering
    \begin{tabular}{c|c|c} 
        \textbf{Parameter} & \textbf{LR inputs} & \textbf{HR targets}  \\
        \hline
        Number of elements & 128 & 128 \\
        Array pitch & 0.3 mm & 0.3 mm \\
        Array aperture & 38.4 mm & 38.4 mm \\
        Transmit Frequency & 4 MHz & 12 MHz \\
        Number of plane waves & 3 ($-10.2^{o}$, $0^{o}$, and $10.2^{o}$) & 75 ($-18^{o}$ to $18^{o}$) \\
        Image reconstruction & pixel-based DAS & pixel-based MV + compounding
        % Sampling Frequency & 25 MHz \\
    \end{tabular}
\label{table:parameters}
\end{table*}

% The training process contained 31 sets of images (465 total images), where each set contains 15 input LR images, and the corresponding target HR image. All images have been compiled using pixel based beamforming. It contains a mix of in-vivo and simulated data, at a ratio of approximately 3:1 (345:120 images). The simulated data is a scan of randomly spaced point scatterers created using the Verasonics simulation mode. 

The training data contains 465 input-target pairs, one input being a stack of 3 LR single PW images, and the target being the corresponding HR image acquired subsequently. It contains a mix of \textit{in-vivo} and \textit{in-silico} data, at a ratio of approximately 3:1 (345 \textit{in-vivo} and 120 \textit{in-silico}). The validation set contains 60 input-target pairs, and the test set contains 45 input-target pairs (30 \textit{in-vivo} and 15 \textit{in-silico}).

In addition to this, due to the increased attenuation of the high-frequency targets, and therefore a lack of SNR at depth, we only include image pixels up to a set depth ($\sim$2.33 cm) for training. In addition, we exclude the first $\sim$0.3 cm, which predominantly consists of ringing. Note that for inference, we evaluate the full depth.  

%with a depth offset, i.e., we skip a few pixels from the shallowest part of our image to de-bias the training. This is important as the shallowest parts of the \textit{in-vivo} images consistently contains artefacts that do not necessarily exist in all kinds on images (for example, \textit{in-silico} images). 
% Thus, by placing a emphasis on the relevant features, we help focus the network towards enhancing the resolution of features using the underlying signal, rather than replicating artefacts that may not always exist. This is a concrete example of GANs 'hallucinating'.

% The validation set contained 4 image sets (60 images), giving a total of 35 image sets. The in-vivo data was collected through 3 separate scan sessions. The test set contains 45 images, 30 in-vivo images and 15 simulated point scatterer images.



==> Deep Proximal Learning for High-Resolution Plane Wave Compounding/chapters/discussion.tex <==
\section{Discussion}\label{chapter:discussion}

% While the network can produce highly denoised predictions for a majority of the frames, it appears to be limited in how much it can potentially denoise the input signal, as seen in \ref{fig:results_image_2}. When the in-vivo input images have a slightly higher magnitude of noise than a certain threshold, the network tends to make predictions of a lower quality. Leading to the hypothesis that it has learnt to denoise the input signal only up to a certain amplitude of noise. The solution to this problem can be as simple as augmenting training data with a larger amplitude of noise. But can also be remedied during deployment by applying a mean filter across adjacent frames. However, to solve the underlying issue at hand, a full sensitivity study is required. 

% Also cleans up the ring down artefact at the top (?) or skin.

% However, it seems to be quite sensitive to the input features themselves. As can be seen with figure \ref{fig:simulated_point}. While the predictions are of good quality, one of the point scatterers is missing from the tailing end of the middle section. This could be attributed to the features themselves being quite unclear in the input images. 


We first start with Fig. \ref{fig:simulated_data}, which makes the distinction between testing the network with \textit{in-silico}, and \textit{in-vivo} samples. Due to the stark differences in the distribution of the images, the variance of the combined test set can be quite high. Therefore, we plot two trend lines, showing that results improve for both \textit{in-vivo} images, and simulated point scatterer data. This indicates that adding \textit{in-silico} data in the training loop can also help improve the quality of not just \textit{in-silico} inputs, but also \textit{in-vivo} data. It also shows that augmenting limited \textit{in-vivo} training data with \textit{in-silico} data is a valid approach. 

Fig. \ref{fig:fwhm_im} shows that the proposed network does indeed improve the beam profile of point scatterers. The network not only manages to improve the lateral localisation of the point scatterer, but also reduces the noise in its periphery, as seen in the input profile and the regularly compounded profile.

While augmenting the \textit{in-vivo} dataset with a sizeable volume of \textit{in-silico} samples improves results, eventually hitting a point of diminishing returns, the same cannot be said of adding folds to the network. In Fig. \ref{fig:unfolded_res}, we show that increasing the number of folds in a network does not necessarily lead to better results. But rather that the optimum number of folds may lay with an intermediary number of unfoldings, which is in line with other works that deal with unfolded networks \cite{solomon2019deep}.

In Fig. \ref{fig:compare_all_res}, we see that the network does succeed in improving the spatial resolution and contrast of the input signal, with the image quality approaching the ground truth. We also have predictions by the benchmark networks compared to the unfolded network shown in Fig. \ref{fig:compare_all_mods}. Although the UNet performs quite well when considering the metrics from Table \ref{table:results}, visually, we see that the results are hazy and undefined. Whereas the CNN is noisy, and is potentially hallucinating the noise that we observe in the predicted image. We can therefore hypothesise that the UNet based networks are perhaps under-specified, and have therefore learnt a shortcut to optimise the problem at hand. While the CNN performs better than the UNet visually, it comes at the cost of a larger computational cost, and a more noticeable noise profile.

A similar effect is in action in Table \ref{table:ablation}, when $\lambda_{1} = 0.0$ (adversarial loss weight term). The MAE for the \textit{in-vivo} samples indicate that the results are better, however, qualitatively/perceptual performance is worse. This is because the adversarial loss tends to promote reconstruction of the high frequency, crisp details of an image, while the $\ell_{1}$ loss is in practice dominated by errors in the low frequency components. Thus, without a perceptual penalty on the sharpness of an image (via the adversary), the resulting image tends to be blurry and hazy. Fig. \ref{fig:comparison_models_3}, in appendix B displays the images that are obtained from networks that have been trained with the $\mathcal{L}_{\ell_{1}}$ and the $\mathcal{L}_{adv}$ components turned off individually. 

% Qualitatively, this indicates that the adversarial loss promotes high-resolution features, while the pixel-wise l1 loss boosts overall contrast

% However, this effect is laid bare when we look into the \textit{in-silico} samples, as it relies on a combination of these terms to obtain the best results, as speckle does not play a role in skewing the result any longer.

While we employ a combination of both pixel-based and distribution-based loss, the neural network optimises for the lowest value of loss, rather than the best visual representation of the US signal data. Although it is advantageous to use such a combination, it presents us with a problem that has been encountered in US imaging before, and demonstrates why it is equally important to visually inspect the resulting images in addition to relying on metrics. More importantly, the benchmark networks lack any of the physics-based design considerations that the proposed network possesses.

% This can partly be explained by the fact that the network optimises for the lowest value of loss, rather than the best visual representation of the signal. Therefore, it is important to also visually verify predictions, in addition to analysing the overall metrics. 

These results allude to the advantages of using model based networks in challenging ill-posed problems, as it appears to promote stability by virtue of its architecture. We also find that it is crucial to transform the output of the unfolded network using an RF-to-Image transformation function (equation \eqref{eq:normer}) before the calculation of the losses (much more trivial to balance loss terms), or passing it on to the discriminator.

% When it comes to the discriminator, this is a crucial step due to our choice of the activation function (LeakyRelu).


% However, the metrics and human perception of a predicted image don't always match up for the networks.

% [As in all data-driven techniques, we learn the free-parameters from data. As such, we expect to deploy this solution in an environment with a similar data distribution.]

==> Deep Proximal Learning for High-Resolution Plane Wave Compounding/chapters/introduction.tex <==
\section{Introduction}\label{chapter:introduction}

\begin{figure*}[t!]
    \centering
    \includegraphics[trim={0 11cm 4 3cm},clip,width=\textwidth]{images/unfolding_figure.pdf}
    \caption{Unfolded deep proximal learning, obtained by unfolding the recurrent proximal gradient scheme to a K layered neural network.}
    \label{fig:network}
\end{figure*}

In Plane Wave (PW) imaging, multiple low resolution images are acquired using steered transmissions, which are then coherently compounded to obtain a high quality image with enhanced lateral resolution and contrast. Compounding more steered plane wave acquisitions improves image quality \cite{tanter2014ultrafast}, but comes at the cost of temporal resolution, i.e. frame-rate. This poses challenges for applications that rely on high frame rates, such as elastography, Ultrasound Localisation Microscopy (ULM) \cite{van2020super}, or sensitive Doppler. One way to improve temporal resolution is to reduce the number of steered PWs transmitted per acquisition, but this negatively impacts lateral resolution. In this paper, we propose a model-based Deep Learning (DL) solution that aims to relax this trade-off between lateral resolution and frame-rate, achieving high resolution and contrast by compounding just 3 PW transmissions.

Deep Learning has revolutionised many domains. It is also increasingly being used in ultrasound based applications \cite{van2019deep, bell2020challenge}. Convolutional Neural Nets (CNNs), such as ResNets \cite{szegedy2017inception} and UNets \cite{ronneberger2015u} have produced excellent results in denoising tasks \cite{wang20183d}. Other applications of Deep Neural Networks (DNNs) in ultrasound include the weighting of channel signals (adaptive beamforming by deep learning) \cite{luijten2020adaptive}, probabilistic sub-sampling for compressed sensing \cite{huijben2019deep}, and coherent PW compounding \cite{gasse2017high}. Related to this work, Gasse et al. (2017) \cite{gasse2017high} use a CNN in tandem with Maxout activation functions, to coherently compound 3 beamformed images, acquired using 1 PW each, and map them towards an image acquired using 31 PWs. Most of the work in the domain of plane wave compounding is achieved by using a variation of the ResNet \cite{khan2019universal} or the UNet architectures \cite{guo2020high}, sometimes in combination with a discriminator in a Generative Adversarial Network-like (GAN) training strategy \cite{zhang2018high, goodfellow2014generative}. There are also works exploring channel-based compounding, in pursuit of better image quality \cite{rothlubbers2020improving}. However, generic convolutional neural networks like a UNet, or a ResNet may sometimes yield solutions that are either physically invalid, or are visually implausible. In other words, they may violate the physical measurement model. Such Neural Networks (NNs) are also typically over-parameterised \cite{cohen2018distribution}. By training light weight models, we tend to limit or avoid the under-specification problem, as there are fewer degrees of freedom in the NN architecture \cite{d2020underspecification, geirhos2020shortcut, cohen2019deep}.

This study expands upon the initial work of \cite{chennakeshava2020high}, by incorporating physics-based inductive biases. We do this by employing physics-based signal priors in the design of our NN, such that we may obtain a network that is compact, yet performs very well when compared to benchmarks (a UNet, ResNet, and \cite{gasse2017high}). In addition, we take further advantage of the signal's noise characteristics in this work. Therefore, this problem is formulated as an ill-posed, linear inverse problem that we solve using data-driven techniques. We achieve an additional boost in the spatial resolution and contrast of the resulting image by training towards images acquired using a higher frequency, and many more PWs. Furthermore, to promote consistency between frames we implement a frame-to-frame loss, which suppresses uncorrelated noise between the frames.

We begin by describing the methods employed in deriving the unfolded proximal gradient descent scheme in Section \ref{chapter:methods}, followed by details about the data acquisition technique, and the volume of data collected in Section \ref{chapter:data_acquisition}. We then describe the training strategy in Section \ref{chapter:training}, and showcase the results in Section \ref{chapter:results}. We discuss the results in Section \ref{chapter:discussion}, and finally conclude the paper in Section \ref{chapter:conclusion}.

% While the in-clinic use of ultrasound (US) for patient monitoring, and intervention is highly established, the same cannot be said about remote/portable US devices. One of the challenges faced by such devices is the limited computational power available to it, and consequently, the spatial and temporal resolution of the acquired images.

% We may attain the required lateral resolution and contrast from coherently compounding multiple plane wave (PW) transmissions. However, the acquisition of multiple PWs for every frame results in a loss of temporal resolution, even though we benefit from enhanced lateral resolution. 

% Ultra-fast ultrasound imaging has enabled a plethora of new ultrasound imaging applications, ranging from localisation microscopy, to shear wave elastography, and beyond. However, there are trade-offs to be taken into consideration, such as that between the lateral resolution and the frame rate of the acquisition.

% formulate a linear inverse, ill-posed problem that we solve using data-driven techniques. 

% These image priors are crucial, as any particular Low Resolution (LR) image can correspond to a set of High Resolution (HR) images: a highly challenging problem which is very sensitive to perturbations in the data. 

%Commonly-used deep neural networks in computer vision, such as ResNets \cite{szegedy2017inception}, Generative Adversarial Networks (GANs) \cite{goodfellow2014generative}, and Convolutional Neural Nets (CNNs) have produced excellent results regarding denoising \cite{wang20183d}, the weighting of PW contributions \cite{luijten2020adaptive}, and coherent PW compounding \cite{gasse2017high}. Related to this work, Gasse et al. (2017) \cite{gasse2017high} use a CNN in tandem with Maxout activation functions, to coherently compound 3 beamformed images, acquired using 1 PW each, and map it towards an image acquired using 31 PWs. Most of the work in this domain is related to plane wave compounding by using a variation of the ResNet \cite{khan2019universal} or the UNet architecture \cite{guo2020high}, sometimes in combination with a discriminator in a GAN like training strategy \cite{zhang2018high}. There are also works exploring channel based compounding, in pursuit of better image quality \cite{rothlubbers2020improving}.


% We solve this problem by formulating it as a linear inverse, ill-posed problem that we solve using data-driven techniques. We employ physics based signal priors in the design of our Neural network (NN), such that we may obtain a network that is compact, yet performs very well when compared to benchmarks. This work adds on to the work done in \cite{chennakeshava2020high}, which is based on a similar principle. However, we take further advantage of the signal characteristics in additional ways with this work.

% We aim to promote robustness by also constraining the training of the NN using known properties of the acquired signal.

% With that in mind, we aim to embed a physical measurement model in the NN architecture, such that the resulting model is compact, yet robust. 


% However, generic convolutional neural networks like a UNet, or a ResNet may sometimes yield solutions that are either physically invalid, or are visually implausible. In other words, they may violate the physical measurement model. Such NNs are also typically over-parameterised \cite{cohen2018distribution}. By training light weight models, we also tend to limit or avoid the under-specification problem, as there are fewer degrees of freedom in the NN architecture \cite{d2020underspecification, geirhos2020shortcut}. With that in mind, we aim to embed a physical measurement model in the NN architecture, such that the resulting model is compact, yet has theoretical guarantees derived from the measurement model. We aim to promote robustness by also constraining the training of the NN using known properties of the acquired signal. Furthermore, we achieve an additional boost in the spatial resolution and contrast of the resulting image by training towards images acquired using a higher frequency, and many more PWs.


% Moreover, we also to aim to improve contrast, by beamforming the target images using Minimum Variance (MV) beamforming. We train our networks in a greedy way \cite{bengio2007greedy}, which is shown to be a much more effective way to train such unfolded algorithms. Additionally, we leverage the redundancy in the signal by utilising the $\ell_{2}$ distance between successive acquisitions, in the denoised network prediction space. As plane wave compounding is typically done in the RF domain, the network also operates in the RF domain. We demonstrated that unfolded networks can perform better than regular neural architectures when data is scarce, by leveraging prior knowledge about the signal.

% DNN fits low frequency stuff first \cite{xu2019frequency}.




==> Deep Proximal Learning for High-Resolution Plane Wave Compounding/chapters/method.tex <==

\begin{figure*}[t!]
% trim={<left> <lower> <right> <upper>}
    \centering
    \includegraphics[trim={0cm 8cm 2cm 3cm},clip,width=\textwidth]{images/overview_figure.pdf}
    \caption{Illustration of data and loss in the training loop. Pink indicates the flow of loss values, and black indicates the flow of data, from input to output. The $U$ blocks indicate the unfoldings of the proximal network, up to $K$ unfoldings. The block to the right hand side of the image with a neuron indicates the discriminator. As we need frame $\textit{t-1}$ and \textit{t} for the calculation of all loss terms, the graphic also displays the training loop across frames in an acquisition.}
    \label{fig:train}
\end{figure*}


\section{Methods}\label{chapter:methods}

% In this work, we consider a set of Low Resolution (LR) images $\mathbf{y}$, which are to be compounded to reconstruct a High Resolution (HR) image $\mathbf{x}$. 

\subsection{Signal model and problem formulation}

\noindent We model the problem of compounding multiple plane waves as an inverse problem in which we aim to recover an underlying high-resolution (HR), high-contrast image from a set of low-resolution (LR) noisy measurements with multiple angled plane waves. We denote $\mathbf{x} \in \mathbb{R}^{N}$ as the vectorised high-resolution beamformed RF image, and $\mathbf{y} \in \mathbb{R}^{NM}$ the vectorised measurement of low-resolution beamformed RF images from $M$ transmitted plane waves. We consider these measurements to be acquired according to the following linear model:
\begin{equation}
    \mathbf{y} = \mathbf{A} \mathbf{x} + \mathbf{n}.
    \label{eq:measurement_model}
\end{equation}
Here,
\begin{equation}
    \mathbf{A} = \begin{pmatrix}\mathbf{A}_{1} \\
    \mathbf{A}_{2} \\
    \vdots \\ \mathbf{A}_{M}\end{pmatrix},
    \label{eq:observation_m}
\end{equation}
and
\begin{equation}
    \mathbf{y} = \begin{pmatrix}\mathbf{y}_{1} \\
    \mathbf{y}_{2} \\
    \vdots \\ \mathbf{y}_{M}\end{pmatrix},
    \label{eq:measured_m}
\end{equation}
where $\mathbf{y}_{m}$ is the vectorised, beamformed RF image belonging to the $m^{\textrm{th}}$ steered plane wave transmission, $\mathbf{n}$ $\in$ $\mathbb{R}^{NM}$ is a noise vector which is assumed to follow a Gaussian distribution with zero mean and diagonal covariance, and $\mathbf{A}$ $\in$ $\mathbb{R}^{NM \times N}$ is a block matrix, with its blocks $\mathbf{A}_{1}$, $\mathbf{A}_{2}$,..., $\mathbf{A}_{M}$ being the measurement matrices of individual PW acquisitions. These measurement matrices capture the transformation between our underlying high-resolution RF image $\mathbf{x}$ and each of the plane wave measurements, and are a function of their respective point spread functions. We assume that they follow a convolutional Toeplitz structure through which we may re-write application of $\mathbf{A}_{M}$ as a convolution with an anisotropic `blurring' kernel. 

Solving equation \eqref{eq:measurement_model} for $\mathbf{x}$ is an ill-posed problem, and hence direct maximum-likelihood estimation may lead to solutions that are not consistent with our prior belief of what HR images look like (anatomical and visual plausibility). To incorporate such priors, we estimate $\mathbf{x}$ through Maximum A-Posteriori (MAP) estimation:
\begin{equation}
    \hat{\mathbf{x}} := \argmax_\mathbf{x} p(\mathbf{x}|\mathbf{y}) \propto \argmax_\mathbf{x} p(\mathbf{y}|\mathbf{x}) p_{\theta}(\mathbf{x}),
    \label{eq:map}
\end{equation}
where $\mathbf{\hat{\mathbf{x}}}$ is the estimated high-resolution ultrasound image, and $p(\mathbf{y}|\mathbf{x})$ is the likelihood according to the linear measurement model in \eqref{eq:measurement_model}, having a Gaussian distribution on the model errors. Here, $p_{\theta}(\mathbf{x})$ is a probability density function that expresses prior beliefs about the distribution of HR images $\mathbf{x}$, where $\theta$ are learnt parameters.

Under a Gaussian model on $p(\mathbf{y}|\mathbf{x})$, taking the log of \eqref{eq:map} results in:
\begin{equation}
    % \hat{\mathbf{x}} = \argmin_\mathbf{x}\norm{\mathbf{y}_{m}-\mathbf{A}_{m}\mathbf{x}}_{2}^{2} + R(\mathbf{x}),
    \hat{\mathbf{x}} = \argmin_\mathbf{x}\norm{\mathbf{y}-\mathbf{A}\mathbf{x}}_{2}^{2} - \log p_{\theta}(\mathbf{x})
    \label{eq:formal_problem}
\end{equation}
where $\log p_{\theta}(\mathbf{x})$ acts as a regulariser $R(\mathbf{x})$ for the optimisation problem.

% When put together with a Laplacian distribution on $\mathbf{x}$, we can re-write equation \ref{eq:formal_problem} as

% \begin{equation}
%     \hat{\mathbf{x}} = \argmin_\mathbf{x}\norm{\mathbf{y}_{m}-\mathbf{A}_{m}\mathbf{x}}_{2}^{2} + \lambda \norm{\mathbf{x}}_{1}
%     \label{eq:formal_problem}
% \end{equation}
% where $\lambda$ is a weight parameter that balances the two terms of the problem statement.

\subsection{Proximal gradient iterations}

Assuming $p_{\theta}(\mathbf{x})$ is given, we proceed by formulating a proximal gradient solver for \eqref{eq:formal_problem}. This results in an iterative algorithm that alternates between a gradient update step with respect to the measurement model (data consistency), and a proximal step that pushes the intermediate solutions in the proximity of the regulariser. One iteration is given by:
\begin{equation}
    \begin{aligned}
        \mathbf{\hat{x}}^{(k+1)} &= \mathcal{P}(\mathbf{\hat{x}}^{(k)}- \mu \mathbf{A}^{T}(\mathbf{A}\mathbf{\hat{x}}^{(k)} - \mathbf{y})),
    \end{aligned}
    \label{eq:iterations}
\end{equation}
where $\mathcal{P}^{(k)}$ is the proximal operator of the regularizer $R(\mathbf{x})$ norm \cite{van2019deep}, and $\mu$ is a step size. We can rewrite \eqref{eq:iterations} in a compact form, separating contributions of $\hat{\mathbf{x}}$ and $\mathbf{y}$, as 
\begin{equation}
    \begin{aligned}
        \mathbf{\hat{x}}^{(k+1)} &= \mathcal{P}_{\theta}^{(k)}(\mathbf{\hat{x}}^{(k)}- \mu^{(k)} \mathbf{A}^{T}(\mathbf{A}\mathbf{\hat{x}}^{(k)} - \mathbf{y})) \\
        &= \mathcal{P}_{\theta}^{(k)}(\mu^{(k)} \mathbf{A}^{T}\mathbf{y}+   (\mathbf{I} - \mu^{(k)} \mathbf{A}^{T}\mathbf{A}) \mathbf{\hat{x}}^{(k)}) \\
        &= \mathcal{P}_{\theta}^{(k)}(\mathbf{W}^{(k)}\mathbf{y}+\mathbf{V}^{(k)}\mathbf{\hat{x}}^{(k)}).
    \end{aligned}
\end{equation}
where we denote $\mathbf{W}^{(k)} = \mu^{(k)} \mathbf{A}^{T}$ and $\mathbf{V}^{(k)} = \mathbf{I} - \mu^{(k)} \mathbf{A}^{T}\mathbf{A}$.

For particular distributions $p_{\theta}(\mathbf{x})$ the proximal operator $\mathcal{P}_{\theta}$ has a closed form. For example, if $p_{\theta}(\mathbf{x})$ is a Laplace distribution, equivalent to $\ell_{1}$ regularisation on $\mathbf{x}$, $\mathcal{P}$ takes the well-known form of a soft-thresholding operator. 


\subsection{Deep unfolding}

In this work, instead of formalising regularizers analytically, we learn the proximal operator directly from an empirical data distribution, similar to \cite{mardani2018neural}. To that end, we unfold the iterations of \eqref{eq:iterations} into a K-layered neural network $U_\theta$, following \cite{gregor2010learning, monga2019algorithm, solomon2019deep} and shown in Fig. \ref{fig:network}. Unfolding allows us to learn both the proximal operator (under some parameterisation $\theta$) and the parameters of the gradient update, $\mathbf{V}^{(k)}$ and $\mathbf{W}^{(k)}$, in an end-to-end fashion.
% Fixed spatial support, and transitionally invariant

Exploiting the block convolutional structure of $\mathbf{A}$, we implement $\mathbf{W}^{(k)}$ as:
\begin{equation}
    \mathbf{W}^{(k)}\mathbf{y} := \mathbf{w}_{1}^{(k)} \circledast \mathbf{y}_{1} + \mathbf{w}_{2}^{(k)} \circledast \mathbf{y}_{2} + ... + \mathbf{w}_{M}^{(k)} \circledast \mathbf{y}_{M},
    \label{eq:seven}
\end{equation}
and, likewise:
\begin{equation}
    \mathbf{V}^{(k)}\mathbf{\hat{x}}^{(k)} = \mathbf{v}^{(k)} \circledast \mathbf{\hat{x}}^{(k)},
    \label{eq:eight}
\end{equation}
where $\circledast$ denotes a convolutional operation, $\lbrace\mathbf{w}_{1}^{(k)}, ..., \mathbf{w}_{M}^{(k)}\rbrace$ and $\mathbf{v}^{(k)}$ are learned convolutional kernels, where we adopted a size of $3\times3$. 

We model $\mathcal{P}_{\theta}^{(k)}$ using a U-Net-style architecture with 9 convolutional layers with Leaky ReLU activations (see Table \ref{table:prox}, in appendix A for architectural details). As mentioned before, making $\mathcal{P}_{\theta}^{(k)}$ trainable avoids the need to devise hand-designed priors with an analytical proximal operator \cite{scherzer1993use}, and instead allows for data-driven proximal mappings that are learned from the training data distribution. As an additional advantage, unrolling the iterative scheme into a fixed-complexity trained computational graph yields a fast solution that avoids the problem of ambiguous computational complexity in iterative algorithms.

% [From ATA matrix to conv kernel]

%, with $\mathbf{A}^{k}$ and $\mathbf{G}^{k}$ being the convolutional kernels ($\mathbf{G}^{k} \approx \mathbf{I} - \mu^{k} \mathbf{A}^{T}\mathbf{A}$). 

%Typically, one would have to hand design a signal prior for the problem at hand, often tuned manually or computed using cross validation \cite{scherzer1993use}. However, we set out to learn the neural proximal mapping using data driven methods, by employing a UNet style network \cite{rick2017one}. This is designated by $\mathcal{P}_{\theta}^{k}$ (a 9 layered CNN with LeakyReLU activations). 

% However, this result only holds when $m$ is small compared to the number of columns in the matrices of $\mathbf{A}_{m}$.

% [] where [] (stacked convolutional) measurement matrix which models the mapping from the HR image $\mathbf{\hat{x}}$ to the low frequency single PW transmit measurements in $\mathbf{y}_{m}$. denotes the neural proximal mapping.

% This is justifiable due to an assumption about the structure of the measurement matrices. Since $\mathbf{A}^{k}$ is assumed to have a sparse toeplitz structure, $\mathbf{G}^{k}$ inherits this assumption as $\mathbf{G}^{k} = \mathbf{I} - \mu^{k} \mathbf{A}^{T}\mathbf{A}$. Here $\mu^{k}$ may be ignored as it only acts as a scaling factor to the term ($\mathbf{A}^{T}\mathbf{A}$). Thus, $\mathbf{A}^{k}$ and $\mathbf{G}^{k}$ may be re-structured as convolutional kernels to facilitate the required convolutional operations. 

% \begin{equation}
%     \mathbf{W}_{2}^{k} = \mathbf{G}^{k} \circledast \mathcal{P}_{\theta}^{k}(\tilde{\mathbf{x}})
%     \label{eq:eight}
% \end{equation}
% \begin{equation}
%     \mathbf{G}^{k} \approx \mathbf{I} - \mu^{k} \mathbf{A}^{T}\mathbf{A}
% \end{equation}

==> Deep Proximal Learning for High-Resolution Plane Wave Compounding/chapters/results.tex <==
\section{Results}\label{chapter:results}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/sim-4.pdf}
    \caption{This figure plots the performance of the proposed network as the volume of \textit{in-silico} data in the training set in increased. The performance on the \textit{in-vivo} and \textit{in-silico} test sets, are shown separately. Notably, \textit{in-vivo} performance improves when adding a significant amount of \textit{in-silico} images to the train set. Due to vast differences in the distributions of \textit{in-silico} and \textit{in-vivo} data, we plot the trends separately such that trend lines are comprehensible for both \textit{in-vivo} and combined test sets.}
    \label{fig:simulated_data}
\end{figure}



\begin{figure}[t!]
    \centering
    \includegraphics[width=0.4\textwidth]{images/fwhm_sim_hil_uncut.pdf}
    \caption{The graphs displays the beam profiles of a point scatterer generated by a \textit{in-silico}, and the subsequent prediction on that data.}
    \label{fig:fwhm_im}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/unfold-4.pdf}
    \caption{The graph displays the relationship between the number of unfoldings in the deep proximal network, and the performance on the test set. Due to vast differences in the distributions of \textit{in-silico} and \textit{in-vivo} data, we plot the trends separately such that trend lines are comprehensible for both \textit{in-vivo} and combined test sets.}
    \label{fig:unfolded_res}
\end{figure}

The results presented in this section were obtained using a network with 5 folds (unless otherwise stated) using the aforementioned framework to construct and train an unfolded proximal gradient network.

% We have as yet presented a method and a framework with which we may construct and train an unfolded proximal gradient network. Using which, we create a network with 5 folds (unless otherwise stated) with which we obtain our results as presented in this section.

The first row of Fig. \ref{fig:compare_all_res} shows the log-compressed and envelope detected input images, obtained using single 4 MHz transmits, along with the corresponding image target acquired using 75 PW transmits at 12 MHz, followed by the compounded image obtained using the proposed method. Perceptually, the resulting image has a similar fidelity as the target, showing high structural resolution and contrast.  

In the second row of Fig. \ref{fig:compare_all_res}, we display the result of our unfolded proximal gradient network when applied to \textit{in-silico} point scatterers, showing strong contrast, resolution, and side-lobe suppression. Fig. \ref{fig:fwhm_im} displays a comparison of the beam profile of a point scatterer, between different methods of beamforming and compounding methods.

Figure \ref{fig:compare_all_mods} show a comparison between the various techniques of compounding the given set of LR images. We compare the resulting images from standard coherent compounding, the target (MV), the prediction by the proposed network, a UNet, and the CNN by Gasse et al. \cite{gasse2017high}. 

Table \ref{table:results} quantifies the Mean Absolute Error (MAE) values, the number of parameters, and the un-optimised inference times of the proposed network (with 5 folds), a UNet-like network (UNet Lite; see Table \ref{table:unet_lite} in appendix A for architectural details) with a similar number of parameters, a full UNet \cite{ronneberger2015u}, and the CNN of \cite{gasse2017high}, containing about 60\% more free parameters than the proposed network. We chose UNets as the benchmark because it is shown to be a very good baseline for such problems \cite{hauptmann2020unreasonable}. Furthermore, most other works rely on a variation of a neural network with skip connections, so the UNet is a good common denominator. This comparison is made on the test data that was gathered for use in this project, as described in Section \ref{chapter:data_acquisition}. The benchmark networks were trained using the same training strategy as the proposed network, albeit not in a greedy training strategy. 

Table \ref{table:ablation} shows the results of an ablation study evaluating the contribution of the individual loss terms in \eqref{eq:final_simplified} to the results. In both Table \ref{table:results} and Table \ref{table:ablation}, we separate the calculation of the MAE between the \textit{in-vivo} and \textit{in-silico} test samples. 

% This is done due to the stark difference in the distribution of the two sets of images, and consequently the difference in the distribution of the predictions made by the networks.

Additionally, we performed experiments to ascertain the volume of \textit{in-silico} data that should be added to the training loop in order to obtain the best performance. Fig. \ref{fig:simulated_data} quantifies the result of such experiments, showing the MAE metric as a function of the number of \textit{in-silico} training data to \textit{in-silico} training data. We also performed an empirical search for the optimal number of layers, and trained the network with 3, 5, 7, and 10 folds. The result of this search is shown in Fig. \ref{fig:unfolded_res}, which displays the MAE metric as a function of the number of unfoldings of the proximal network. 

% \begin{table}[htbp]
% \caption{The table displays a comparison made between the Unfolded Proximal Gradient Scheme, U-Net Lite (a network similar number of parameters), and the CNN published by Gasse et al. (2017).}
% \centering
%     \begin{tabular}{c|c|c} 
%         \hline
%         \multirow{2}*{\textbf{Network}} & \multirow{2}*{\textbf{In-Silico}} & \textbf{No. of} \\
%          &  & \textbf{Parameters} \\
%         \hline
        
%         Unfolded Proximal & \multirow{2}*{0.43 $\pm$ 0.13} & \multirow{2}*{$\sim$ 175 k} \\
%         Gradient Scheme &  &  \\
        
%         UNet Lite & 0.4 $\pm$ 0.08 & $\sim$ 160 k \\
        
%         CNN by & \multirow{2}*{0.36 $\pm$ 0.12} & \multirow{2}*{$\sim$ 280 k} \\
%         Gasse et al. (2017) &  &  \\
%     \end{tabular}
% \label{table:results}
% \end{table}

\begin{table*}[htbp]
\caption{The table displays a comparison made between the proposed Unfolded Proximal Gradient Scheme, U-Net Lite (a network with a similar number of parameters), a full UNet, and the CNN published by Gasse et al. (2017). We compare the Mean Absolute Error (MAE) (including mean and variance across images in the test set), the number of parameters, and inference times (tested on an NVIDIA 3080 Ti).}
\centering
    \begin{tabular}{c|c|c|c|c} 
        \multirow{2}*{\textbf{Network}} & \multicolumn{2}{|c|}{\textbf{Mean Absolute Error (mean $\pm$ var)}} & \textbf{No. of} & \textbf{Inference} \\\cline{2-3}
         & In-Vivo & In-Silico & \textbf{Parameters} & \textbf{Time} \\ 
        \hline
        Unfolded Proximal & \multirow{2}*{1.1$\times 10^{-1}$ $\pm$ 2.6$\times 10^{-4}$} & \multirow{2}*{7.1$\times 10^{-3}$ $\pm$ 1.48$\times 10^{-6}$} & \multirow{2}*{$\sim$ 175 k} & \multirow{2}*{$\sim$ 20 ms} \\
        Gradient &  &  &  & \\
        
        UNet & 1.16$\times 10^{-1}$ $\pm$ 9.8$\times 10^{-8}$ & 1.1$\times 10^{-2}$ $\pm$ 9.7$\times 10^{-7}$ & $\sim$ 1175 k & $\sim$ 8 ms \\
        
        UNet Lite & 1.34$\times 10^{-1}$ $\pm$ 1.93$\times 10^{-3}$ & 1.5$\times 10^{-2}$ $\pm$ 4.94$\times 10^{-6}$ & $\sim$ 160 k & $\sim$ 6 ms \\
        
        CNN by & \multirow{2}*{1.4$\times 10^{-1}$ $\pm$ 1.96$\times 10^{-3}$} & \multirow{2}*{1.8$\times 10^{-2}$ $\pm$ 5.65$\times 10^{-6}$} & \multirow{2}*{$\sim$ 280 k} & \multirow{2}*{$\sim$ 6 ms}\\
        Gasse et al. (2017) &  &  &  & \\
    \end{tabular}
\label{table:results}
\end{table*}

\begin{table*}[htbp]
\caption{The following table shows an ablation study, evaluating the contribution of loss terms as given in equation \eqref{eq:final_simplified}. We present the Mean Absolute Error (MAE), reporting both its mean and standard deviation across the test set.}
\centering
    \begin{tabular}{c|c|c|c|c|c} 
        \multicolumn{3}{c|}{\textbf{Losses}} & \textbf{Training} & \multicolumn{2}{c}{\textbf{Mean Absolute Error (mean $\pm$ var)}} \\ 
        \hline
        Pixel-based distance & Adversary & Frame-to-Frame & & In-Vivo & In-Silico \\ 
        \hline
        \checkmark & \checkmark & \checkmark & Greedy & 1.1$\times 10^{-1}$ $\pm$ 2.6$\times 10^{-4}$ & 7.1$\times 10^{-3}$ $\pm$ 1.48$\times 10^{-6}$
        \\
        - & \checkmark & \checkmark & Greedy & 1.3$\times 10^{-1}$ $\pm$ 1.03$\times 10^{-3}$ & 7.4$\times 10^{-3}$ $\pm$ 1.18$\times 10^{-6}$
        \\
        \checkmark & - & \checkmark & Greedy & 1.03$\times 10^{-1}$ $\pm$ 4.79$\times 10^{-4}$ &7.34$\times 10^{-3}$ $\pm$ 1.16$\times 10^{-6}$
        \\        
        \checkmark & \checkmark & - & Greedy &1.12$\times 10^{-1}$ $\pm$ 2.48$\times 10^{-4}$ & 7.43$\times 10^{-3}$ $\pm$ 1.19$\times 10^{-6}$

    \end{tabular}
\label{table:ablation}
\end{table*}


% [Graphs showing difference in quality of point scatterer prediction, in relation to the proportion of point scatterer images in the training set.]

% [Discussion about the disappearing points]

% [Graphs show comparison between different unfolding numbers.]

% [Plot against how many images you need to compound to get similar performance]

We also re-trained the network after the initial greedy training process, but received no appreciable increase in the quantitative or qualitative metrics of the consequent results.

==> Deep Proximal Learning for High-Resolution Plane Wave Compounding/chapters/training.tex <==
\section{Training Strategy}\label{chapter:training}

% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=\textwidth]{images/gabor_0_2.jpg}
%     \caption{Log-compressed and envelope-detected set of 3 \textit{in-vivo} low-frequency input images, followed by the high frequency ground truth compounded using 75 plane waves and the deep network output. The depicted anatomy is a longitudinal profile at the point of bifurcation of the carotid artery. These images have been taken from the test set.}
%     \label{fig:results_image_1}
% \end{figure*}

% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=\textwidth]{images/gabor_1_sim_2.jpg}
%     \caption{Log-compressed and envelope-detected set of 3 \textit{in-silico} low frequency input images, followed by the high frequency ground truth compounded using 75 plane waves and the deep network output. These images have been taken from the test set.}
%     \label{fig:simulated_point}
% \end{figure*}

\begin{figure*}[t!]
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/gabor_0_2.jpg}
        % \caption{}
        \label{fig:results_image_1}
    \end{subfigure}
    \vfill
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[trim={0cm 0cm 0cm 8.8cm},clip,width=\textwidth]{images/gabor_1_sim_2.jpg}
        % \includegraphics[width=\textwidth]{images/gabor_1_sim_2.jpg}
        % \caption{}
        \label{fig:simulated_point}
    \end{subfigure}
    \caption{Log-compressed and envelope-detected set of 3 \textit{in-vivo} (first row) and \textit{in-silico} (second row) low-frequency input images, followed by the corresponding high frequency ground truth, compounded using 75 plane waves, and the deep network output. The first row depicts a longitudinal profile at the point of bifurcation of the carotid artery. All images were taken from the test set.}
    \label{fig:compare_all_res}
\end{figure*}


In this section, the training strategy is described in detail. To promote high fidelity in the image domain, we guide the optimization by adding an RF-to-image transformation function, $\mathcal{Q}$, to the computational graph before computing the losses. This way we emphasise a high resolution image in the image domain, after envelope detection and log-compression. We define $\mathcal{Q}$ as:
\begin{equation}
    \mathcal{Q}(\mathbf{x}) = 20\log_{10} \left(\epsilon + \frac{|Hilbert(\mathbf{x})|}{\max(|Hilbert(\mathbf{x})|)}\right),
    \label{eq:normer}
\end{equation} 
where $\epsilon$ is a small constant, and the values are clipped outside the range of interest (-60dB to 0dB). We combine 3 loss functions that capture various aspects of desired outputs: a pixel-wise distance loss, an adversarial loss, and a frame-to-frame loss (see Fig. \ref{fig:train} for an overview). 

% The $k^{th}$ fold is always left unfrozen, during this process. 
 %It is also worth noting that the log compression was performed on data with a range of [$\delta$, \textit{max}(\textit{x})]. 
\subsection{Pixel-Based Distance Loss}

We start with a pixel-based distance loss, which computes the average per-pixel $\ell_{1}$ distance between the reconstructed image $\mathcal{Q}(\hat{\mathbf{x}})= \mathcal{Q}(U_\theta(\mathbf{y}_t))$, and the target image $\mathcal{Q}(\mathbf{x})$: 
\begin{equation}
    \begin{aligned}
    \mathcal{L}_{\ell_{1}} &= \mathbb{E}_{(\mathbf{y}, \mathbf{x}) \sim p_{data}} \norm{\mathcal{Q}(\mathbf{x}_{t}) - \mathcal{Q}(U_\theta(\mathbf{y}_{t}))}_{1}
    \end{aligned}
\end{equation}
where $t$ indicates the frame number. Although we have framed the above in terms of expectation values, in practice, we approximate it by sampling a fixed dataset, i.e., the training data.

\subsection{Adversarial Loss}

We also include an adversarial loss to promote perceptually adequate outputs. Such adversaries are often used in GANs: deep generative models trained in a min-max game to map simple Gaussian-distributed noise vectors into outputs that follow a desired target distribution (e.g. an empirical distribution of natural images). Here we use a similar setup, and train our deep unfolded proximal gradient network in a min-max game with a neural adversary to produce outputs that, given the particular input data, fall within the distribution of high-resolution ultrasound images as sampled in our training set. By not just assessing outputs but rather input-output pairs, we mitigate hallucination of output image features that fall within the distribution of HR images, but are not consistent with the input data. 

%However, we use a variant of the GAN called a Conditional GAN (CGAN)\cite{mirza2014conditional}, where the observed image $\mathbf{y}$ and the random noise $\mathbf{z}$ is mapped to the target image $\mathbf{x}$, $G(\mathbf{y}, \mathbf{z})$ $\rightarrow$ $\mathbf{x}$. 

Our neural adversary, $D_\psi$, outputs its belief that the image data spanned by its receptive field belongs to the set of high-resolution images. Here, $D_\psi$ is fully convolutional and has a receptive field smaller than the image dimensions (see Table \ref{table:discriminator}, in appendix A for architectural details), thus outputting probabilities for multiple distinct image regions (i.e. like a patchGAN \cite{isola2017image}). This directs the focus of the adversary towards local image quality features, rather than global semantic features. 

% However, we use a variant of the GAN called a conditional GAN (CGAN), where both the generator and discriminator are conditioned on some extra information $\mathbf{x}$. Which leads us to $G(\mathbf{z}|\mathbf{x})$ $\rightarrow$ $\mathbf{\hat{x}}$.

We train $D_\psi$ by minimizing the binary cross-entropy classification loss between its predictions and the labels (target or generated), evaluated on batches that contain both target images and generated images. At the same time, the deep compounding network $U_\theta$ is trained to maximize this loss, thereby attempting to fool the adversary. This leads to the following optimization problem across the training data distribution $p_{data}$:

% \begin{multline}

%     \hat{\theta},\hat{\bm{\Psi}} =  \underset{\mathbb{\psi}}{\mathrm{argmax}}~ \underset{\mathbb{\theta}}{\mathrm{argmin}}
%     \Bigr\{-\mathcal{L}_{adv}\Bigr\}\ \\ =\underset{\mathbb{\psi}}{\mathrm{argmax}}~ \underset{\mathbb{\theta}}{\mathrm{argmin}}
%     \Bigr\{\mathbb{E}_{(\mathbf{y}_t,\mathbf{x}_t)\sim p_{data}}\left[
%             \log(D_{\psi}(\left[\mathcal{Q}(\mathbf{y}_t),\mathcal{Q}(\mathbf{x}_t)\right]))+ \right. \\ \left. \log(1-D_{\psi}(\left[\mathcal{Q}(\mathbf{y}_t),\mathcal{Q}(U_\theta(\mathbf{y}_t))\right]))
%             \right]\Bigr\},
            
%     \label{eqn:optimization_adversary}
% \end{multline}


\begin{multline}
    \begin{aligned}
        \hat{\theta}, \hat{\mathbb{\psi}} &= \argmax_{\mathbb{\psi}} \argmin_{\mathbb{\theta}} \left\{-\mathcal{L}_{adv}\right\} \\
        &= \argmax_{\mathbb{\psi}} \argmin_{\mathbb{\theta}} \mathbb{E}_{(\mathbf{y}_{t},\mathbf{x}_{t})\sim p_{data}} \\ &\qquad \left\{\log(D_{\psi}([\mathcal{Q}(\mathbf{y}_{t}),\mathcal{Q}(\mathbf{x}_{t})])) + \right. \\ & \left. \qquad \qquad \log(1-D_{\psi}([\mathcal{Q}(\mathbf{y}_{t}), \mathcal{Q}(U_\theta(\mathbf{y}_{t}))]))\right\},
    \end{aligned}
    \label{eqn:optimization_adversary}
\end{multline}
where $\theta$ are the parameters of the compounding network and $\psi$ are the parameters of the discriminator $D_\psi$. 

% \begin{equation}
%     L(G,D) = \mathbb{E}_{\mathbf{y},\mathbf{x}} log D(\mathbf{y}|\mathbf{x}) + \mathbb{E}_{\mathbf{y},\mathbf{z}} log(1-D(G(\mathbf{z}|\mathbf{x})))
% \end{equation}


% We achieve this by using the Binary Cross Entropy.

% \begin{equation}
%     BCE = - (\mathbf{y}_{t} log(p(\hat{x}_{t})) + \\
%     (1-\mathbf{y}_{t}) log(1-p(\hat{x}_{t}))) 
% \end{equation}
% where $p(\hat{x}_{t})$ represents the probability that ($\hat{x}_{t}$) was sampled from 


% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=\textwidth]{images/comparison_models_1t.jpg}
%     \caption{This figure compares different compounding methods against the target. We compare our approach against standard coherent compounding, compounding by a UNet, and the architecture proposed by Gasse \textit{et al.} in \cite{gasse2017high}. The anatomy is a longitudinal profile at the point of bifurcation of the carotid artery. These images have been taken from the test set.}
%     \label{fig:comparison_models}
% \end{figure*}

% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=\textwidth]{images/comparison_models_2.jpg}
%     \caption{This figure compares different compounding methods against the target. We compare our approach against standard coherent compounding, compounding by a U-Net, and the architecture proposed by Gasse \textit{et al.} in \cite{gasse2017high}. The anatomy is a longitudinal profile of the carotid artery. These images have been taken from the test set.}
%     \label{fig:comparison_models_2}
% \end{figure*}

\begin{figure*}[t!]
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/comparison_models_1t.jpg}
        % \caption{}
        \label{fig:comparison_models}
    \end{subfigure}
    \vfill
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[trim={0cm 0cm 0cm 8.8cm},clip,width=\textwidth]{images/comparison_models_2.jpg}
        % \includegraphics[width=\textwidth]{images/comparison_models_2.jpg}
        % \caption{}
        \label{fig:comparison_models_2}
    \end{subfigure}
    \caption{This figure compares different compounding methods against the target. We compare our approach against standard coherent compounding, compounding by a U-Net, and the architecture proposed by Gasse \textit{et al.} in \cite{gasse2017high}. The first row depicts a longitudinal profile of the carotid artery at the point of bifurcation. The second row depicts a longitudinal profile of the carotid artery. All images were taken from the test set.}
    \label{fig:compare_all_mods}
\end{figure*}

\subsection{Frame-to-Frame Loss}

In addition to the $\ell_{1}$ distance, and the adversarial loss mentioned above, we also implement an $\ell_{2}$ distance on consecutive frames ($(t-1)^{th}$ and $t^{th}$ frame) as predicted by $U_\theta$. This is done to promote consistency between frames while suppressing (frame-wise) uncorrelated noise:
% This helps promote consistency of predictions between consecutive frames, and reduce prediction noise.
% The training strategy also involves a frame-to-frame penalty, which we achieve by passing frame $(t-1)$ through the network, followed by the second frame $(t)$. This is then followed by taking the $\ell_{2}$ distance between the two frames as predicted by $G$. This is done to promote consistency between frames while suppressing (frame-wise) uncorrelated noise. 
\begin{equation}
    \mathcal{L}_{ftf} = \mathbb{E}_{(\mathbf{y}_{t}, \mathbf{y}_{t-1}) \sim p_{data}} \norm{\mathcal{Q}(U_\theta(\mathbf{y}_{t-1})) - \mathcal{Q}(U_\theta(\mathbf{y}_{t}))}_{2}^{2} .
\end{equation}


\subsection{Training details and parameters}
% does appear to provide higher quality, and robust results. 

% We use a combination of pixel based (mean absolute error), and distribution based based losses \cite{isola2017image}. 

%With the loss functions now defined, we may now focus on the training pipeline. The input to such a pipeline are the sets of three beamformed images ($\mathbf{y}_{t-1}$ and $\mathbf{y}_{t}$), acquired at PW steering angles of $-10.2^{o}$, $0^{o}$, and $10.2^{o}$. Which are then compounded towards a high resolution target gathered using 75 PW transmissions.

% Here, we learn all of the free parameters from data. We train the network end-to-end with 5 unfoldings of the Unfolded Proximal Gradient Network, using a combination of mean absolute error and perceptive losses \cite{isola2017image}. We leverage a staggered loss strategy, in which the loss after each fold, $k$, is weighted by an exponentially increasing factor. The training strategy also contains a discriminator block (a four layered CNN with LeakyReLU activations), which when taken together with the unfolded iterative scheme, forms the full training pipeline. The input to this network is a set of three beamformed images, beamformed using PWs steered at $-10.2^{o}$, $0^{o}$, and $10.2^{o}$ respectively, acquired at 4 MHz. This is then trained towards a ground truth image beamformed and compounded using 75 PWs at 12 MHz, corresponding to steering angles between $-18^{o}$ and $18^{o}$. 

%Deviating from the regular CGAN structure slightly, the discriminator in our work takes in the three input images, and the the target/prediction as a stacked input. This provides the discriminator with an additional mapping between the LR inputs and the HR targets/predictions, so that the unfolded network may get a higher quality feedback from the discriminator. 

The total loss function is a weighted sum of the aforementioned losses, and given by:
\begin{equation}
    \mathcal{L}_{tot} = \lambda_{1} \cdot \mathcal{L}_{adv} + \lambda_{2} \cdot \mathcal{L}_{\ell_{1}} + \lambda_{3} \cdot \mathcal{L}_{ftf}
    \label{eq:final_simplified}
\end{equation}
where $\lambda_{i}$ are weight terms, with $\lambda_{1} = 1.0$, $\lambda_{2} = 1.0$, and $\lambda_{3} = 0.001$ in our experiments, determined empirically.

We train the network in a greedy manner \cite{bengio2007greedy, belilovsky2019greedy}, i.e. fold-by-fold. In the first iteration, we only train the first fold. We then add the next fold, freezing the first, and continue training. This process continues until all folds are trained. Note that the last convolutional layer of the architecture (see Fig. \ref{fig:train}) is trained in every iteration. Each fold is trained for 1800 epochs, with a batch size of 1. We use the Adam optimiser \cite{kingma2014adam} with a learning rate of $1 \times 10^{-5}$, and with a $\beta_{1} = 0.5$. All other optimiser parameters are left at default, as described in \cite{kingma2014adam}.

All of the networks were created using Python 3 and TensorFlow 2 \cite{tensorflow2015-whitepaper}, and trained using an NVIDIA 2080 Ti GPU. 

% where BCE is the Binary Cross Entropy, MAE is the Mean Absolute Error, and the MSE is the Mean Square Error, which is implemented at point of prediction between successive frames.
% \begin{multline}
%     L = \frac{1}{n} \sum_{i=1}^{n} \Big[ - \lambda_{1} \cdot  (y_{i, t} log(p_{i, t}) + \\
%     (1-y_{i, t}) log(1-p_{i, t})) \\
%     + \lambda_{2} \cdot |y_{i, t} - x_{i, t}| \\
%     + \lambda_{3} \cdot (y_{i, t-1} - y_{i, t})^{2} \Big]
% \end{multline}
% where n is the training batch size, y is the prediction, and x is the label. 

% \begin{multline}
%     L = \frac{1}{n} \sum_{i=1}^{n} \Big[ \lambda_{1} \cdot  BCE \{ \mathcal{Q}(y_{i, t}), \mathcal{Q}(x_{i, t}) \} \\
%     + \lambda_{2} \cdot MAE \{ \mathcal{Q}(y_{i, t}), \mathcal{Q}(x_{i, t}) \} \\
%     + \lambda_{3} \cdot MSE \{ \mathcal{Q}(y_{i, t-1}), \mathcal{Q}(y_{i, t}))^{2} \} \Big]
% \end{multline}

% \begin{multline}
%     L =  \lambda_{1} \cdot \arg \min_{G} \max_{D} \mathcal{Q}(L(G,D)) + \\ \lambda_{2} \mathbb{E}_{\mathbf{y}, \mathbf{x}, \mathbf{z}} \norm{\mathcal{Q}(\mathbf{x}_{t}) - \mathcal{Q}(\hat{\mathbf{x}}_{t})}_{1} + \\
%     \lambda_{3} \cdot \mathbb{E}_{\mathbf{y}, \mathbf{z}} \norm{\mathcal{Q}(\hat{\mathbf{x}}_{t-1}) - \mathcal{Q}(\hat{\mathbf{x}}_{t})}_{2}^{2}
% \end{multline}


%Where $0^{+}$ indicates a quantity that is slightly greater than $0$, i.e., $(0 + \delta)$.

% However, if we are considering envelope detected data, we simply only perform the log compression, without the Hilbert transform, as described by,

% \begin{multline}
%     L = \frac{1}{n} \sum_{i=1}^{n} \Big[ \lambda_{1} \cdot  BCE \{ log_{10}(y_{i, f+1}), log_{10}(x_{i, f+1}) \} \\
%     + \lambda_{2} \cdot MAE \{ log_{10}(y_{i, f+1}), log_{10}(x_{i, f+1}) \} \\
%     + \lambda_{3} \cdot MSE \{ log_{10}(y_{i, f}), log_{10}(y_{i, f+1}))^{2} \} \Big]
% \end{multline}
% and subsequently dropping the noise components.

%This is done under the assumption that the key features do not change drastically between subsequent frames, allowing us the opportunity to exploit that information. 

%Resulting in a smoother and more consistent prediction across all input frames in a particular movie.

%Unfolded networks are typically very tricky to train, along with being difficult to replicate. 

% We further constrain the network by employing a staggered loss strategy, where the loss at the $k^{th}$ fold is weighted with an exponentially increasing factor. Such a factor was determined empirically. 

% We also use a discriminator block in the training pipeline (a four layered CNN with LeakyReLU activations).

% We also find that it is crucial to transform the output of the unfolded network using equation \ref{eq:normer} before the calculation of the losses (much more trivial to balance loss terms), or passing it on to the discriminator. When it comes to the discriminator, such a step is crucial due to our choice of activation function. 
% This enhances the resolution of features, which was otherwise lacking.

% This step seem crucial due to an interplay between the generator and the discriminator, and are not fully clear as to why it makes such a large difference. Perhaps it is due to a "squaring effect", where image pixel values, when raised to the $n^{th}$ power, sharpens select features.


%We also wrote a Hilbert transform using TensorFlow functions to be compatible with TensorFlow's graph mode.


